ByteComposer: a Human-like Melody Composition Method based on Language Model Agent

Large Language Models (LLM) have shown encouraging progress in multimodal understanding and generation tasks. However, how to design a human-aligned and interpretable melody composition system is still under-explored. To solve this problem, we propose ByteComposer, an agent framework emulating a human's creative pipeline in four separate steps : "Conception Analysis - Draft Composition - Self-Evaluation and Modification - Aesthetic Selection". This framework seamlessly blends the interactive and knowledge-understanding features of LLMs with existing symbolic music generation models, thereby achieving a melody composition agent comparable to human creators. We conduct extensive experiments on GPT4 and several open-source large language models, which substantiate our framework's effectiveness. Furthermore, professional music composers were engaged in multi-dimensional evaluations, the final results demonstrated that across various facets of music composition, ByteComposer agent attains the level of a novice melody composer.

==> 1.method.v1.tex <==

% \cite{relevant_paper_for_generator}
% \cite{relevant_paper_for_voter}

\subsection{Prompt Design}

Although LLMs have been demonstrated to be powerful few-shot learners across various tasks, their capabilities can only be fully unleashed through carefully designed prompts tailored to the desired behavior. The quality of the generated output is often sensitive to design choices in the prompt, sometimes down to the selection of punctuation marks. To this end, we identify core components of the prompts and evaluate different design choices through cross-validation. Detailed evaluations of key design decisions will be discussed in Section x. We ultimately classify prompts into two categories: process-related prompts and music theory-related prompts.

\begin{enumerate}
    \item \textbf{Process-Related Prompts:} To ensure the smooth operation of the entire workflow, the first step involves the design of appropriate process prompts. Clear and logical context cues guide the LLM to understand its current state and complete tasks within the current workflow accordingly.
    
    \item \textbf{Music Theory-Related Prompts:} To stimulate the LLM's music theory knowledge and enhance the quality of music generation, we design prompts specifically related to music theory:
    \begin{enumerate}
        \item \textbf{Music Theory Explanation:} Explicit explanations of music theory attributes are included within the prompt.
        
        \item \textbf{Music Attribute Guidance:} By listing musical attributes, the LLM is guided to select those most congruent with the theme of the generation.
        
        \item \textbf{Few-Shot Learning:} Specific examples are provided for the LLM to reference.
    \end{enumerate}
\end{enumerate}

% Citation placeholder
% \cite{relevant_paper_for_prompt_design}
\subsection{Expert Module}

The ByteComposer system's heartbeat is the Expert module, an intricate segment that intertwines multiple layers of music generation with finesse. More than just a component, the Expert module acts as the central orchestrator, setting the rhythm and tone for the entire musical composition journey.

The module's journey starts with the conceptualization and arrangement phase. Drawing insights from user inputs, it analyzes the interplay between user preferences, musical traditions, and contemporary composition techniques. The aim here is clear: to create a musical roadmap that captures the artist's intent and resonates with the audience's expectations.

In its next phase, the module actively collaborates with a plethora of music generation tools. Think of the Expert module as a master conductor, tapping into various sections of an orchestra, ensuring each contributes its unique flavor to the overall composition. It's not merely calling tools to action but ensuring their contributions harmonize to produce a unified musical piece.

This leads to the critical stage of score evaluation. The Expert module, with its vast reservoir of musical knowledge, assesses each composition with precision. By offering objective metrics, benchmarked against global standards, coupled with nuanced subjective insights, it ensures every potential deviation from perfection is noted. This feedback is not just about finding flaws but charting a path for potential enhancements.

In ensuring the composition's seamless journey, the Expert module employs a vigilant state routing mechanism. Depending on the current node's status and guided by insights from the Memory module, it either propels the composition forward or, if needed, revisits previous stages, ensuring a solid foundation.

% Citation placeholder
% \cite{relevant_paper_for_expert_module}

\subsection{Implementation of the Expert Module}

The Expert module stands on the technological bedrock of LLMs combined with the strategic use of robust prompts. Several leading models, including ChatGPT, GPT-4, and LLama2, are harnessed, especially when paired with Few-Shot Prompting, allowing for a diverse exploration of musical terrains.


A significant underpinning of the Expert module's success lies in its data-driven approach. A meticulously curated set of approximately 90,000 prompts, synergized with GPT-based models, set the stage for an expansive musical landscape. The emphasis on SFT further solidified the LLM's capabilities, making the ByteComposer pipeline even more resilient and efficient.



% Citation placeholder
% \cite{relevant_paper_for_implementation}


\subsection{Generator Module}
\subsubsection{Functionality}
\begin{enumerate}
    \item Attribute-Controlled Generation: The Generator can produce music based on specified attributes.
    \item Local Modifications: A bar-level similar score generation module has been designed to implement local error corrections or rewriting capabilities.
\end{enumerate}

\subsubsection{Implementation}
\begin{enumerate}
    \item GPT-4: Directly employs the ABC notation generation capabilities inherent in GPT-4.
    \item TunesFormer Plus:
    \begin{enumerate}
        \item Utilizes the dataset from TunesFormer with added musical attributes and employs GPT-2 as the backbone.
        \item Designs a bar-level similar score generation module to improve local modification capabilities.
    \end{enumerate}
\end{enumerate}

\subsection{Voter Module}
\subsubsection{Functionality}
\begin{enumerate}
    \item The model aims to align with human preferences to select the most pleasing compositions when no objective errors are found.
\end{enumerate}

\begin{figure}
    \centering
    \includegraphics{figures/expert_voter.pdf}
    \caption{Professionally Rendered Trio Score with Rich Information.}
\end{figure}

\subsubsection{Implementation}
\begin{enumerate}
    \item GPT-4: Direct utilization of GPT-4 outputs.
    \item Llama2-Qlora-SFT:
    \begin{enumerate}

